AbPress: Flexing Partial-Order Reduction and Abstraction

Partial-order reduction (POR) and lazy abstraction with interpolants are two complementary techniques that have been successfully employed to make model checking tools for concurrent programs effective. In this work, we present AbPress - Abstraction-based Partial-order Reduction with Source-Sets - an algorithm that fuses a recently proposed and powerful dynamic POR technique based on source-sets and lazy abstraction to obtain an efficient software model checker for multi-threaded programs. It trims the inter- leaving space by taking the abstraction and source-sets into account. We amplify the effectiveness of AbPress with a novel solution that summarizes the accesses to shared variables over a collection of interleavings. We have implemented AbPress in a tool that analyzes concurrent programs using lazy abstraction, viz., Impara. Our evaluation on the effectiveness of the presented approach has been encouraging. AbPress compares favorably to existing state-of-the-art tools in the landscape.

==> covers-bg.tex <==
\subsection {Covers with POR}

In a recent work \cite{wko2013}, a combination of Impact algorithm 
with POR was presented. Addition of POR enabled the verifier 
to detect that a certain schedules will merge in future. 
%
Impact with covers alone can't discover this information in 
advance. Thus, POR technique in combination with covers
offer a more robust technique in addressing the state-space 
explosion during the process of verification.
%




